Quantum One-Time Memories from Stateless Hardware, Random Access Codes, and Simple Nonconvex Optimization

We present a construction of one-time memories (OTMs) using classical-accessible stateless hardware, building upon the work of Broadbent et al. and Behera et al.. Unlike the aforementioned work, our approach leverages quantum random access codes (QRACs) to encode two classical bits, $b_0$ and $b_1$, into a single qubit state $\mathcal{E}(b_0 b_1)$ where the receiver can retrieve one of the bits with a certain probability of error. To prove soundness, we define a nonconvex optimization problem over POVMs on $\mathbb{C}^2$. This optimization gives an upper bound on the probability of distinguishing bit $b_{1-\alpha}$ given that the probability that the receiver recovers bit $b_\alpha$ is high. Assuming the optimization is sufficiently accurate, we then prove soundness against a polynomial number of classical queries to the hardware.

==> sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this work, we presented a construction of one-time memories (OTMs) using stateless hardware.
\LEV{TODO!!}





==> sections/conj_unlock.tex <==
\newcommand{\statePl}{\ket{+}\bra{+}}
\newcommand{\stateMi}{\ket{-}\bra{-}}

\section{Wiesner States and Unlocking Oracles}

We will take a slightly different approach from Ref.~\cite{broadbent2021towards} in proving secure one-time memories.
First, we will use two-seperate oracles for $s_+$ and $s_\times$: $\orac_+ = \Obf[C_+], \orac_\times = \Obf[C_\times]$ \LEV{TODO defn somewhere}.
Then, treating the harware-tokens as VBB obfuscations, we can note that if the min-entropy of an accepting input to $\orac_b$ is high, then the oracle is \emph{indistinguishable} from the null-oracle.
Thus, prior to making any accepting calls to $\orac_+$ or $\orac_\times$, the simulator can use a null-oracle instead.
Next, we (heuristically using non-convex optimization) show that for $\advers$ to learn an accepting input on, WLOG, $\orac_+$, the trace distance between $\statePl$ and $\stateMi$ must be non-trivially below $1$ and thus the min-entropy of an accepting string to $\orac_\times$ must be high!

\begin{figure}
	\begin{mdframed}
		$C_{\theta}(M)$ for $M \in \set{0, 1}^n$ and hardcoded values $\theta \in \set{+, \times}$ and secret $r_\theta, p_\theta \in \set{0, 1}^n$
		\begin{itemize}
			\item If $M[p_\theta] = r_\theta$, output $s_\theta$
			\item Otherwise, output $\bot$
		\end{itemize}
	\end{mdframed}
	\caption{Lockable Circuit for $s_\theta$}
\end{figure}

\begin{figure}
	\begin{mdframed}
		Prepare one-time memory:
		\begin{itemize}
			\item Samples $p_+ \randomGets \in \set{0, 1}^n$,
				let $p_\times = \overline{p_+}$, $r_+, r_\times \randomGets \set{0, 1}^{|p_+|}$,
				and $r_\times \randomGets \set{0, 1}^{|p_\times|}$
		\item Sample $s_\theta \in \set{0, 1}^n$
			\item Let $\orac_\theta \gets \Obf[C_\theta]$ for $\theta \in \set{+, \times}$
			\item Return $\ket{\psi} = \bigotimes_{i \in [n]} \ket{b_i}^{\theta_i}, \orac_+, \orac_\times$ where 
				\[
					\begin{cases}
						\theta_i = + \text{ if } p_+[i] = 1 \\
						\theta_i = 0 \text{ otherwise}
					\end{cases}
				\]
				and
				\[
					\begin{cases}
						b_i = r_+[i] \text{ if } \theta_i = +\\
						b_i = r_\times[i] \text{ otherwise }
					\end{cases}
				\]
		\end{itemize}
		Measure $(\ket{\psi}, \orac_+, \orac_\times, \alpha \in \set{+, \times})$
		\begin{itemize}
			\item Measure in basis $\alpha$ to get $M' \in \set{0, 1}^n$
			\item Return $\orac_\alpha(M')$
		\end{itemize}
	\end{mdframed}
	\caption{One Time Memory Protocol}
\end{figure}


\subsubsection*{Proof}
WLOG we will show that if $\advers$ can learn an accepting input to $\orac_+$, then the min-entropy of an accepting input to $\orac_\times$ is high.

\begin{lemma}[Adversary Decomposition]
	For (quantum) PPT adversary, $\calA$, if there exists quantum PPT $M_+, \aux_1 \gets \calA_1(\Obf[0], \ket{\psi}), \calA_2(M_\times, M_+, \aux_1, \orac_+, \orac_\times)$ such that
	\[
		\calA \compInd \calA_2 \circ \calA_1
	\]
	and there does not exist $\calA_2'(M_\times, M_+, \aux_1, \Obf[0])$ such that
	\[
		\calA \compInd \calA_2' \circ \calA_1
	\]
	\LEV{TODO: fix notation here... with comp}
	then \[
		\Pr[M_+' \text{ accepts} \mid M_+' \gets \calA'(M_+)] \geq 0.95^n
	\]
	% TODO: define $A_+$ as accepting state and this as min-guessing prob?
	% TODO accepts, actual numbers, etc
\end{lemma}
\begin{proof}
	\LEV{TODO}
\end{proof}

\begin{lemma}[Independence Prior to Unlock]



\end{lemma}

\begin{lemma}[Indepedence Prior to Unlock]
	\[
		\HMax(A_+ \mid \Obf[0], \ket{\psi}) = \sum_{i \in [n]} \HMax(A^i_+ \mid \Obf[0], \ket{\psi})
	\]
\end{lemma}



We will prove simulation-secure one-time memories and show how to prove security in the quantum UC in appendix \LEV{TODO: and justify why}.j

\LEV{TODO: Quantum UC model :*P???? Maybe needed for quantum OTMs which is sad... fix later... proof in appendix to boost to Quantum UC}





==> sections/obf.tex <==

\LEV{How formal does this need to be?}
%
%\begin{definition}[Classical Forcing]
%	Let $C$ be some classical circuit, we then let its classically forced circuit be the following quantum circuit:
%	\[
%		\CF{C}(\ket{\psi}) = C(\mu_Z(\ket{\psi}))
%	\]
%	where $\mu_Z$ is measurement in the $Z$ basis.
%\end{definition}
%
%
%We slightly change the definition of virtual black box obfuscation from Ref.~\cite{bartusek2019new} to incorperate ``classical forcing''.
%\begin{definition}[Classical Query Virtual Black Box Obfuscation]
%	\begin{enumerate}
%		\item Strong Functionality Preservation: For every $n \in \N$, $C \in \calC_n$, there exists a neglible function $\eps$ such that
%			\[
%				\Pr[\Obf(C, 1^n)(\ket{\psi}) = \CF{C}(\ket{\psi}) \; \forall \ket{\psi} \in \C^{2^n}] = 1 - \eps(n).
%			\]
%		\item Polynomial Slowdown: For every $n \in \N$ and $C \in \calC_n$, the evaluation of $\Obf(C, 1^n)$ is polynomially slower than the evaluation of $C$.
%		\item Distributional Virtual Black-Box: For every PPT adversary $\advers$, there exists a (non-uniform) polynomial size simulator $\Sim$ such that for every \(n \in \N\), every distribution \(D \in \mathcal{D}_n\) (a distribution over \(C_n\)), and every predicate \(P: C_n \to \{0, 1\}\), there exists a negligible function \(\mu\) such that
%			\[
%				\left| 
%				\Pr_{C \leftarrow \calD_n} \left[ \advers(\text{Obf}(C, 1^n)) = P(C) \right] - 
%				\Pr_{C \leftarrow \calD_n} \left[ \Sim^{\CF{C}}(1^{|C|}, 1^n) = P(C) \right] 
%				\right| = \mu(n).
%			\]
%	\end{enumerate}
%\end{definition}

